Instance-Level Data-Use Auditing of Visual ML Models

The growing trend of legal disputes over the unauthorized use of data in machine learning (ML) systems highlights the urgent need for reliable data-use auditing mechanisms to ensure accountability and transparency in ML. We present the first proactive, instance-level, data-use auditing method designed to enable data owners to audit the use of their individual data instances in ML models, providing more fine-grained auditing results than previous work. To do so, our research generalizes previous work integrating black-box membership inference and sequential hypothesis testing, expanding its scope of application while preserving the quantifiable and tunable false-detection rate that is its hallmark. We evaluate our method on three types of visual ML models: image classifiers, visual encoders, and vision-language models (Contrastive Language-Image Pretraining (CLIP) and Bootstrapping Language-Image Pretraining (BLIP) models). In addition, we apply our method to evaluate the performance of two state-of-the-art approximate unlearning methods. As a noteworthy second contribution, our work reveals that neither method successfully removes the influence of the unlearned data instances from image classifiers and CLIP models, even if sacrificing model utility by $10\%$.

==> discussion.tex <==
\section{Discussion} \label{sec:discussion}


\subsection{Auditing Other Types of Data} \label{sec:discussion:text_data}

Our work mainly focuses on image instance auditing. While our method could be generalized into
other types of data, such as text data, such generalization presents several challenges. A key difficulty 
lies in generating $\NumberMarkedData$ distinct marked instances for each raw data sample. 
Taking text data as example, previous works have proposed methods of generating marked text data 
by adding random sequence~\cite{wei2024:proving}, substituting characters with their lookalike characters~\cite{wei2024:proving}, 
or paraphrasing~\cite{huang2024:auditdata}. However, marked text data created by appending random sequences or 
using lookalike character substitutions can often be easily recovered to the original text without 
compromising data utility. Paraphrasing-generated marked data is also vulnerable to adversary's evading 
detection by re-paraphrasing it. Also, it is challenging to paraphrase a raw text data for
$\NumberMarkedData$ times to generate $\NumberMarkedData$ distinct marked text data while
ensuring that all of them preserve the semantic meaning.

